Implementing packet trimming support in hardware

Packet trimming is a primitive that has been proposed for datacenter networks: to minimize latency, switches run small queues; when the queue overflows, rather than dropping packets the switch trims off the packet payload and either forwards the header to the destination or back to the source. In this way a low latency network that is largely lossless for metadata can be built. Ideally, trimming would be implemented as a primitive in switch ASICs, but hardware development cycles are slow, costly, and require demonstrated customer demand. In this paper we investigate how trimming can be implemented in existing programmable switches which were not designed with trimming in mind, with a particular focus on a P4 implementation on the Tofino switch ASIC. We show that it is indeed possible to closely approximate idealized trimming and demonstrate that trimming can be integrated into a production-grade datacenter switch software stack.

==> figures/simulator/3-to-1-worst/plot <==
set term pdfcairo font "Helvetica,20"

set output "3-to-1-worst.pdf"
set xlabel "Tims (ms)"
set ylabel "Throughput (Gbps)"

plot "f1" using ($1*1000):($13*8/1000000000) w l t "Flow 1",\
     "f2" using ($1*1000):($13*8/1000000000) w l t "Flow 2",\
     "f3" using ($1*1000):($13*8/1000000000) w l t "Flow 3"


==> figures/simulator/4-to-1-worst/plot <==
set term pdfcairo font "Helvetica,20"

set output "4-to-1-worst.pdf"
set xlabel "Time (ms)"
set ylabel "Throughput (Gbps)"

plot "f1" using ($1*1000):($13*8/1000000000) w l t "Flow 1",\
     "f2" using ($1*1000):($13*8/1000000000) w l t "Flow 2",\
     "f3" using ($1*1000):($13*8/1000000000) w l t "Flow 3",\
     "f4" using ($1*1000):($13*8/1000000000) w l t "Flow 4"


==> figures/simulator/mechanism_comparison/16-1/plot <==
set term pdfcairo font "Helvetica,22"

set output "16to1.pdf"
#set xrange [-250:]
set key left top

set xlabel "Header seqno compared to highest seen"
set ylabel "CDF"

plot "out_tofino_dod.cdf" using 1:($0/65.2) w l lw 3 t "DoD", \
     "out_tofino_full.cdf" using 1:($0/66.42) w l lw 3 t "Full",\
     "out_tofino_ideal.cdf" using 1:($0/65.24) w l lw 3 t "Ideal",\
     "out_tofino_mod.cdf" using 1:($0/65.2) w l lw 3 t "MOD"

set output "16to1_time.pdf"
set key right bottom

set grid

unset xrange
#set logscale x 2

set xlabel "Header receive time (us)"
set ylabel "CDF"
set yrange [0:100]

plot      "out_tofino_ideal_time.cdf" using ($1*1000):($0/65.24) w l lw 5 dt 1 lc rgb "black" t "Ideal",\
     "out_tofino_full_time.cdf" using ($1*1000):($0/66.4) w l lw 3 dt 1 lc rgb "red" t "Tofino",\
     "out_tofino_dod_time.cdf" using ($1*1000):($0/65.2) w l lw 5 dt 2 lc rgb "blue"  t "DoD", \
     "out_tofino_mod_time.cdf" using ($1*1000):($0/65.2) w l lw 5 dt 4 lc rgb "gray" t "MOD"

==> figures/simulator/mechanism_comparison/4-1/plot <==
set term pdfcairo font "Helvetica,22"

set output "4to1.pdf"
set xrange [-250:]
set key left top

set xlabel "Header seqno compared to highest seen"
set ylabel "CDF"
set yrange [0:100]

plot "out_tofino_dod.cdf" using 1:($0/60.64) w l lw 3 t "DoD", \
     "out_tofino_full.cdf" using 1:($0/71.90) w l lw 3 t "Full",\
     "out_tofino_ideal.cdf" using 1:($0/60.80) w l lw 3 t "Ideal",\
     "out_tofino_mod.cdf" using 1:($0/60.64) w l lw 3 t "MOD"

set output "4to1_time.pdf"
set key left top

set grid

#set logscale x 2

unset xrange
set xrange [:25]
#set xtics (0.125, 0.5,1,2,4,8,16,32,64,128,256)

set xlabel "Header receive time (us)"
set ylabel "CDF"
set yrange [0:100]


plot      "out_tofino_ideal_time.cdf" using ($1*1000):($0/60.8) w l lw 5 dt 1 lc rgb "black" t "Ideal",\
     "out_tofino_full_time.cdf" using ($1*1000):($0/71.56) w l lw 3 dt 1 lc rgb "red" t "Tofino",\
     "out_tofino_dod_time.cdf" using ($1*1000):($0/60.64) w l lw 5 dt 2 lc rgb "blue"  t "DoD", \
     "out_tofino_mod_time.cdf" using ($1*1000):($0/60.64) w l lw 5 dt 4 lc rgb "gray" t "MOD"

#     "out_tofino2_time.cdf" using ($1*1000):($0/61.51) w l lw 3 t "Tofino2"
     

==> figures/simulator/mechanism_comparison/64-1/plot <==
set term pdfcairo font "Helvetica,22"

set output "64to1.pdf"
set key left top

set xlabel "Header seqno compared to highest seen"
set ylabel "CDF"
set yrange [0:100]

plot "out_tofino_dod.cdf" using 1:($0/7.63) w l lw 3 lt -1 t "DoD", \
     "out_tofino_full.cdf" using 1:($0/7.63) w l lw 3 lt 0 t "Tofino",\
     "out_tofino_ideal.cdf" using 1:($0/7.63) w l lw 3 lt 1 t "Ideal",\
     "out_tofino_mod.cdf" using 1:($0/7.57) w l lw 3 lt 2 t "MoD"

set output "64to1_time.pdf"
set key right bottom


unset xrange
#set logscale x 2
set grid

set xlabel "Header receive time (us)"
set ylabel "CDF"
set yrange [0:100]

plot      "out_tofino_ideal_time.cdf" using ($1*1000):($0/6.3) w l lw 5 dt 1 lc rgb "black" t "Ideal",\
     "out_tofino_full_time.cdf" using ($1*1000):($0/6.36) w l lw 3 dt 1 lc rgb "red" t "Tofino",\
     "out_tofino_dod_time.cdf" using ($1*1000):($0/6.29) w l lw 5 dt 2 lc rgb "blue"  t "DoD", \
     "out_tofino_mod_time.cdf" using ($1*1000):($0/6.29) w l lw 5 dt 4 lc rgb "gray" t "MOD"
#     "out_tofino2_time.cdf" using ($1*1000):($0/6.29) w l lw 3 t "Tofino2"

==> figures/simulator/mechanism_comparison/8-1/plot <==
set term pdfcairo font "Helvetica,20"

set output "8to1.pdf"
#set xrange [-250:]
set key left top

set xlabel "Header seqno compared to highest seen"
set ylabel "CDF"

plot "out_tofino_dod.cdf" using 1:($0/63.68) w l lw 3 t "DoD", \
     "out_tofino_full.cdf" using 1:($0/69.03) w l lw 3 t "Full",\
     "out_tofino_ideal.cdf" using 1:($0/63.76) w l lw 3 t "Ideal",\
     "out_tofino_mod.cdf" using 1:($0/63.68) w l lw 3 t "MOD"

set output "8to1_time.pdf"
set key right bottom

set grid

unset xrange
#set logscale x 2

set xlabel "Header receive time (us)"
set ylabel "CDF"
set yrange [0:100]

plot "out_tofino_dod_time.cdf" using ($1*1000):($0/63.68) w l lw 3 t "DoD", \
     "out_tofino_full_time.cdf" using ($1*1000):($0/69.03) w l lw 3 t "Full",\
     "out_tofino_ideal_time.cdf" using ($1*1000):($0/63.76) w l lw 3 t "Ideal",\
     "out_tofino_mod_time.cdf" using ($1*1000):($0/63.68) w l lw 3 t "MOD"


==> space-tricks.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}

%\usepackage[small,compact,noindentafter]{titlesec} 
\usepackage[compact]{titlesec}

\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}

%\usepackage[inline]{enumitem}
%\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=0pt,skip=0pt,font={stretch=0.9}]{caption}
%\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}

%\titleformat{\subsection}
%  {\normalfont\fontsize{12}{15}\bfseries}{\thesection}{1em}{}

